Experimental Realization of a Reconfigurable Electroacoustic Topological Insulator

A substantial challenge in guiding elastic waves is the presence of reflection and scattering at sharp edges, defects, and disorders. Recently, mechanical topological insulators have sought to overcome this challenge by supporting back-scattering resistant wave transmission. In this Letter, we propose and experimentally demonstrate the first \emph{reconfigurable electroacoustic} topological insulator exhibiting an analog to the quantum valley Hall effect (QVHE). Using programmable switches, this phononic structure allows for rapid reconfiguration of domain walls and thus the ability to control back-scattering resistant wave propagation along dynamic interfaces for phonons lying in static and finite-frequency regimes. Accordingly, a graphene-like Polyactic Acid (PLA) layer serves as the host medium, equipped with periodically arranged and bonded piezoelectric patches, resulting in two Dirac cones at the $K-$points. The PZT patches are then connected to negative capacitance external circuits to break inversion symmetry and create nontrivial topologically-protected bandgaps. As such, topologically protected interface waves are demonstrated numerically and validated experimentally for different predefined trajectories over a broad frequency range.

==> defs.tex <==
% This is file JFM2esam.tex
% first release v1.0, 20th October 1996
%       release v1.01, 29th October 1996
%       release v1.1, 25th June 1997
%       release v2.0, 27th July 2004
%   (based on JFMsampl.tex v1.3 for LaTeX2.09)
% Copyright (C) 1996, 1997 Cambridge University Press

\NeedsTeXFormat{LaTeX2e}

%\documentclass{jfm}

\usepackage{mathrsfs}
\usepackage{graphicx}
%\usepackage{natbib}
\usepackage{amsmath}
\usepackage{epstopdf}
\usepackage{color}
\usepackage{soul}
\def\red{\textcolor{red}}
\def\blue{\textcolor{blue}}
\definecolor{darkblue}{RGB}{83,0,93}
\newcommand{\q}[1]{\textcolor{darkblue}{#1}}



%%% Example macros (some are not used in this sample file) %%%

% For units of measure
\newcommand\dynpercm{\nobreak\mbox{$\;$dyn\,cm$^{-1}$}}
\newcommand\cmpermin{\nobreak\mbox{$\;$cm\,min$^{-1}$}}

% Various bold symbols
\providecommand\bnabla{\boldsymbol{\nabla}}
\providecommand\bcdot{\boldsymbol{\cdot}}
\newcommand\biS{\boldsymbol{S}}
\newcommand\etb{\boldsymbol{\eta}}

% For multiletter symbols
\newcommand\Real{\mbox{Re}} % cf plain TeX's \Re and Reynolds number
\newcommand\Imag{\mbox{Im}} % cf plain TeX's \Im
\newcommand\Rey{\mbox{\textit{Re}}}  % Reynolds number
\newcommand\Pran{\mbox{\textit{Pr}}} % Prandtl number, cf TeX's \Pr product
\newcommand\Pen{\mbox{\textit{Pe}}}  % Peclet number
\newcommand\Ai{\mbox{Ai}}            % Airy function
\newcommand\Bi{\mbox{Bi}}            % Airy function
% For sans serif characters:
% The following macros are setup in JFM.cls for sans-serif fonts in text
% and math.  If you use these macros in your article, the required fonts
% will be substitued when you article is typeset by the typesetter.
%
% \textsfi, \mathsfi   : sans-serif slanted
% \textsfb, \mathsfb   : sans-serif bold
% \textsfbi, \mathsfbi : sans-serif bold slanted (doesnt exist in CM fonts)
%
% For san-serif roman use \textsf and \mathsf as normal.
%
\newcommand\ssC{\mathsf{C}}    % for sans serif C
\newcommand\sfsP{\mathsfi{P}}  % for sans serif sloping P
\newcommand\slsQ{\mathsfbi{Q}} % for sans serif bold-sloping Q

% Hat position
\newcommand\hatp{\skew3\hat{p}}      % p with hat
\newcommand\hatR{\skew3\hat{R}}      % R with hat
\newcommand\hatRR{\skew3\hat{\hatR}} % R with 2 hats
\newcommand\doubletildesigma{\skew2\tilde{\skew2\tilde{\Sigma}}}
%       italic Sigma with double tilde

% array strut to make delimiters come out right size both ends
\newsavebox{\astrutbox}
\sbox{\astrutbox}{\rule[-5pt]{0pt}{20pt}}
\newcommand{\astrut}{\usebox{\astrutbox}}

\newcommand\GaPQ{\ensuremath{G_a(P,Q)}}
\newcommand\GsPQ{\ensuremath{G_s(P,Q)}}
\newcommand\p{\ensuremath{\partial}}
\newcommand\tti{\ensuremath{\rightarrow\infty}}
\newcommand\kgd{\ensuremath{k\gamma d}}
\newcommand\shalf{\ensuremath{{\scriptstyle\frac{1}{2}}}}
\newcommand\sh{\ensuremath{^{\shalf}}}
\newcommand\smh{\ensuremath{^{-\shalf}}}
\newcommand\squart{\ensuremath{{\textstyle\frac{1}{4}}}}
\newcommand\thalf{\ensuremath{{\textstyle\frac{1}{2}}}}
\newcommand\Gat{\ensuremath{\widetilde{G_a}}}
\newcommand\ttz{\ensuremath{\rightarrow 0}}
\newcommand\ndq{\ensuremath{\frac{\mbox{$\partial$}}{\mbox{$\partial$} n_q}}}
\newcommand\sumjm{\ensuremath{\sum_{j=1}^{M}}}
\newcommand\pvi{\ensuremath{\int_0^{\infty}%
  \mskip \ifCUPmtlplainloaded -30mu\else -33mu\fi -\quad}}

\newcommand\etal{\mbox{\textit{et al.}}}
\newcommand\etc{etc.\ }
\newcommand\eg{e.g.\ }

\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}

%Some mathematical Definitions
\def\o{\over}
\def\p{\partial}
\def\be{\begin{eqnarray}}
\def\ee{\end{eqnarray}}
\def\bes{\begin{subeqnarray}}
\def\ees{\end{subeqnarray}}
\def\k{\kappa}
\def\o{\omega}
\def\f{\frac}
\def\lp{\left(}
\def\rp{\right)}
\def\lb{\left[}
\def\rb{\right]}
\def\lcb{\left\{}
\def\rcb{\right\}}
\def\n{\nabla}
\def\W{\textbf{W}}
\def\Q{\textbf{Q}}
\def\lap{\nabla^2}
\def\z{\zeta}
\def\ep{\epsilon}
\def\vep{\varepsilon}
\def\r{\rho}
\def\g{\gamma}
\def\t{\times}
\def\l{\lambda}
\def\befi{\begin{figure}}
\def\eefi{\end{figure}}
\def\a{\alpha}
\def\no{\noindent}
\def\bce{\begin{center}}
\def\ece{\end{center}}
\def\ra{\rightarrow}
\def\lra{\longrightarrow}
\def\h{\hat{}}
\def\RA{\rightarrow}
\def\d{\delta}
\def\D{\Delta}
\def\th{\theta}
\def\G{\Gamma}
\def\det{\text{det}}
\def\L{\Lambda}
\def\T{\Theta}
\def\b{\beta}
\def\x{\textbf{x}}
\def\d{\textrm{d}}
\def\n{\nabla}
\def\F{\textbf{F}}
\def\GG{\textbf{G}}
\def\nn{\textbf{n}}
\def\i{\textrm{i}}
\def\ul{\underline}
\def\ba#1\ea{\begin{align}#1\end{align}}
\def\e{\textbf{e}}

\def\bsa#1\esa{\begin{subequations}
\begin{align}#1\end{align} \end{subequations}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "apssamp"
%%% End:
\usepackage{graphicx}% Include figure files
\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{bm}% bold math
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\def\blue{\textcolor{blue}}                                                     
\def\red{\textcolor{red}}                                                       
\def\green{\textcolor{green}}                                                   
\def\black{\textcolor{black}}                                                   
\def\cyan{\textcolor{cyan}}                                                     
\definecolor{darkblue}{RGB}{83,0,93}                                            
\def\L{\large{\textbf{\mbox{------}}}}           
\def\dashL{\large{\textbf{\mbox{-~-~-}}}}               
\def\dotL{\large{\textbf{\mbox{$\cdot\ \cdot\ \cdot$}}}}
\def\cdashL{\large{\textbf{\mbox{--~-~--}}}}
\def\cdotL{\mbox{--- $\cdot$ ---}}                                              
\def\ccdotL{\mbox{--- $\cdot\ \cdot$ ---}}                                      
\def\longdashL{\mbox{--~--~--}}                                                 
\def\zz{($...$)\ }                                                              
\def\dashdot{\mbox{- $\cdot$ -}}                                                
\def\magenta{\textcolor{magenta}}                                               
\def\blue{\textcolor{blue}}                                                     
\def\red{\textcolor{red}}                                                       
\def\green{\textcolor{green}}                                                   
\def\black{\textcolor{black}}                                                   
\def\cyan{\textcolor{cyan}}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{hyperref}% add hypertext capabilities
%\usepackage[mathlines]{lineno}% Enable numbering of text and display math
%\linenumbers\relax % Commence numbering lines

%\usepackage[showframe,%Uncomment any one of the following lines to test
%%scale=0.7, marginratio={1:1, 2:3}, ignoreall,% default settings
%%text={7in,10in},centering,
%%margin=1.5in,
%%total={6.5in,8.75in}, top=1.2in, left=0.9in, includefoot,
%%height=10in,a5paper,hmargin={3cm,0.8in},
%]{geometry}

